SafeCoEvo: Co-Evolving Safety Harnesses and Guards for LLM Agents at Test-Time

LLM agents deployed in real-world environments continually encounter new tasks and safety risks, while execution feedback typically becomes available only after each task is completed. However, existing self-evolving approaches commonly rely on multiple rounds of optimization over fixed and repeatedly accessible task distributions, fundamentally differing from test-time adaptation in real-world deployment, where only experience accumulated from past tasks can be used to improve safety decisions on future unseen tasks. To address this limitation, we propose SafeCoEvo, a test-time Harness-Guard co-evolution framework for LLM agent safety that enables the external safety system to continually adapt from accumulated runtime experience. SafeCoEvo jointly improves two complementary safety capabilities at different timescales: S-Harness rapidly externalizes recent runtime experience into updatable explicit safety knowledge that can promptly influence subsequent tasks, while GuardVPO internalizes accumulated runtime safety experience over a longer timescale into parametric risk-judgment capabilities. By combining short-term rapid adaptation with long-term capability consolidation, SafeCoEvo continually improves the agent's safety capabilities, reducing the unsafe outcome rate by 10.05% while improving the task success rate by 12.15% over the strongest baseline, thereby achieving simultaneous gains in safety and task utility.

==> image/prompt_preamble.tex <==
% Load once in the main document preamble (before \begin{document}).
\usepackage[T1]{fontenc}
\usepackage{url}
\usepackage{listings}
\usepackage{tcolorbox}
\tcbuselibrary{skins,breakable,listings}

\lstdefinestyle{safecoevoprompt}{
  language={},
  basicstyle=\ttfamily\footnotesize,
  columns=fullflexible,
  keepspaces=true,
  breaklines=true,
  breakatwhitespace=false,
  breakautoindent=true,
  breakindent=1em,
  showstringspaces=false,
  showspaces=false,
  showtabs=false,
  tabsize=2,
  numbers=none,
  aboveskip=0pt,
  belowskip=0pt,
  upquote=true
}

\newcommand{\SafeCoEvoPromptFile}[2]{%
  \tcbinputlisting{
    enhanced jigsaw,
    breakable,
    listing only,
    listing engine=listings,
    listing options={style=safecoevoprompt},
    listing file={#2},
    colback=black!3!white,
    colframe=black!28!white,
    colbacktitle=black!8!white,
    coltitle=black,
    fonttitle=\bfseries\small,
    title={#1},
    title after break={#1 (continued)},
    boxrule=0.4pt,
    arc=1mm,
    left=2mm,right=2mm,top=1.5mm,bottom=1.5mm,
    before skip=8pt,after skip=10pt,
    pad at break*=1mm
  }%
}

